Expert Decision Support System for aeroacoustic source type identification using clustering

This paper presents an Expert Decision Support System for the identification of time-invariant, aeroacoustic source types. The system comprises two steps: first, acoustic properties are calculated based on spectral and spatial information. Second, clustering is performed based on these properties. The clustering aims at helping and guiding an expert for quick identification of different source types, providing an understanding of how sources differ. This supports the expert in determining similar or atypical behavior. A variety of features are proposed for capturing the characteristics of the sources. These features represent aeroacoustic properties that can be interpreted by both the machine and by experts. The features are independent of the absolute Mach number which enables the proposed method to cluster data measured at different flow configurations. The method is evaluated on deconvolved beamforming data from two scaled airframe half-model measurements. For this exemplary data, the proposed support system method results in clusters that mostly correspond to the source types identified by the authors. The clustering also provides the mean feature values and the cluster hierarchy for each cluster and for each cluster member a clustering confidence. This additional information makes the results transparent and allows the expert to understand the clustering choices.

==> ExpertDecisionSupportSystem JASA rev2/spectra_prep.tex <==

\section{Spectra preparation}\label{sec:source_identification}
The proposed expert decision support system is based on the feature calculation from source spectra. We obtain these spectra either from single source measurements or from measuring multiple sources at the same time with beamforming~\citep{Beamforming2019} using either manually defined ROIs or using automatic source identification methods such as SIND~\citep{Goudarzi2021}. For the data presented in this paper, we use SIND to obtain the source positions and source spectra.\\

\subsection{Spectra interpolation}
We apply a preprocessing step before calculating features based on the spectra: the spectra are interpolated onto a logarithmic Strouhal and Helmholtz frequency vector. Thus, a discrete bin of the frequency vector represents a constant frequency interval ratio. This ensures that each frequency interval is equally weighted for the calculation of the corresponding features. Also, we will compare spectra over Strouhal and Helmholtz number bin-wise, which requires interpolation to align the frequency bins at different Mach numbers.

\subsection{Source spectra separation}\label{sec:spectra_seperation}
Source spectra can exhibit multiple different source mechanisms in different frequency intervals, either because of complex source mechanisms or simply because a ROI or single measurement contained multiple sources that a super-positioned in the spectra. To calculate correct features based on which the sources can be clustered, we first need to separate the sources which feature multiple mechanisms into sub-sources that only contain the corresponding partial spectrum. This step has to be carried out before the feature calculation, so the feature-set presented in this paper cannot be used to detect this behavior. Thus, we focus on an easily detectable characteristic that many source spectra with multiple mechanisms exhibit. We found that often, a spectrum scales at low frequencies over Strouhal number and at high frequencies over Helmholtz number or vice versa. Thus, there exist two different aeroacoustic mechanisms. We use this observation in the following to identify and separate the spectra accordingly.\\

Consequently, we cut each source spectrum into two sub-spectra and calculate the mean broadband self-similarity (see subsection~\ref{sec:similarity}) for four cases:
\begin{enumerate}
\itemsep-0.1em 
	\item For the Strouhal number at low and high frequencies.
	\item For the Strouhal number at low and the Helmholtz number at high frequencies. 
	\item For the Helmholtz number at low and the Strouhal number at high frequencies. 
	\item For the Helmholtz number at low and high frequencies.
\end{enumerate}
Figure~\ref{fig:Figure01} $c)$ shows the resulting mean self-similarity for different cut-frequencies for a slat / slat track source of the Do728. We calculate the Strouhal number cut-frequency using the mean Mach number $\text{St}=\text{He}/\langle M_i\rangle$. The global optimum of the four cases defines the optimal cut frequency and the frequency types of the sub-spectra. In this case, we achieve the optimal self-similarity when we use the Strouhal number at low frequencies (Figure~\ref{fig:Figure01} $a$, below the vertical black line) and the Helmholtz number at high frequencies (Figure~\ref{fig:Figure01} $b$ above the vertical black line). However, often it is not clear (even for a human) if the spectrum should be separated and a false positive separation has a greater impact on the feature calculation and clustering than a false negative separation. Hence, we prefer to leave a spectrum intact if the need for separation is unclear. We define a variety of rules that must be met before the source is separated into sub-sources. First, the overlapping spectra at different Mach numbers must cover at least two octaves to prevent small sub-spectra with little information. Second, the sub-spectra should both cover at least half an octave to prevent small, irrelevant spectra parts. Third, we only separate the source if the optimal similarity is achieved using a different scaling behavior at low and high frequencies. Forth, the mean self-similarity of the sub-spectra of different frequency-types must feature at least a $\SI{10}{\percent}$ improvement over the maximum mean self-similarity of the same frequency types. In the example of the slat / slat track, the first three rules are met, but the self-similarity improvement of around $\SI{7}{\percent}$ from $\text{He}_\text{cut}(\langle\text{St}_l,\text{He}_h\rangle)\approx14$ would not justify the spectrum separation, compared to sub-spectra with a Helmholtz number scaling at $\text{He}_\text{cut}(\langle\text{He}_l,\text{He}_h\rangle)\approx24$. The parameters for the rules are based on the presented data and can be adjusted to meet a more or less rigorous separation policy.

\begin{figure}
	\centering
	\includegraphics[width=\reprintcolumnwidth]{Figure01}
	\caption{(Color online) Do728, $\text{Re}=\SI{1.4e6}{}$, slat / slat track source at $\alpha=\SI{1}{\degree}$. $a)$ shows the spectra over Strouhal and $b)$ over Helmholtz number. The vertical black lines depict the optimal frequency to separate the spectra into low $l$ and high $h$ sub-spectra, to ensure their optimal self-similarity. In $c)$ the mean self-similarity (scal), see eq.~\ref{eq:scalability}, for the four possible combinations of Strouhal $\text{St}_{l,h}$ and Helmholtz number $\text{He}_{l,h}$ based on the depicted spectra cut-frequency on the x-axis are shown. The $x$ marks the global maximum, which leads to the spectra separation in $a)$ and $b)$. For this source, a Strouhal number scaling below $\text{He}\approx15$ and Helmholtz number scaling above this frequency achieves the optimal self-similarity of the sub-spectra.}
	\label{fig:Figure01}
\end{figure}



% In sub-section~\ref{sec:spectra_seperation} we showed that spectra often contain frequency intervals, that are governed by different physical mechanisms. While we observed most of the characteristic features at lower Strouhal numbers $\text{St}\le 100$, some sources showed a different behavior at high Strouhal numbers, see Figure~\ref{fig:Figure03}. For this, we identified the inner slat, slat / slat tracks, slat edge and the nacelle vicinity, see Figure~\ref{fig:Figure01}, Figure~\ref{fig:Figure03}, and Figure~\ref{fig:Figure07} $a)$, $j)$, $k)$ and $n)$. We showed that this behavior can be detected using the definition of the self-similarity over Strouhal and Helmholtz number from sub-section~\ref{sec:similarity}. We assumed that if a spectrum scales at low frequencies over Strouhal number and at high frequencies over Helmholtz number or vice versa, it must be governed by two different source mechanisms. Thus, the source spectra can be separated into sub-spectra that feature a single source mechanism, respectively. Since a false positive separation of a spectrum can lead to the insufficient calculation of aeroacoustic properties we introduced rules to ensure a conservative spectrum separation policy. The variables of these rules were based on the spectra of the presented datasets and should be reviewed for other data. The sources in our data showed mostly one or two different frequency regions, but more complex sources might be possible. Since we had to manually classify all individual sources for a ground truth and interpret the clustering results, we chose not to complicate the process by splitting spectra. However, the clustering results may be improved using this technique.\\

==> spectra_prep.tex <==

\section{Spectra preparation}\label{sec:source_identification}
The proposed expert decision support system is based on the feature calculation from source spectra. We obtain these spectra either from single source measurements or from measuring multiple sources at the same time with beamforming~\citep{Beamforming2019} using either manually defined ROIs or using automatic source identification methods such as SIND~\citep{Goudarzi2021}. For the data presented in this paper, we use SIND to obtain the source positions and source spectra.\\

\subsection{Spectra interpolation}
We apply a preprocessing step before calculating features based on the spectra: the spectra are interpolated onto a logarithmic Strouhal and Helmholtz frequency vector. Thus, a discrete bin of the frequency vector represents a constant frequency interval ratio. This ensures that each frequency interval is equally weighted for the calculation of the corresponding features. Also, we will compare spectra over Strouhal and Helmholtz number bin-wise, which requires interpolation to align the frequency bins at different Mach numbers.

\subsection{Source spectra separation}\label{sec:spectra_seperation}
Source spectra can exhibit multiple different source mechanisms in different frequency intervals, either because of complex source mechanisms or simply because a ROI or single measurement contained multiple sources that a super-positioned in the spectra. To calculate correct features based on which the sources can be clustered, we first need to separate the sources which feature multiple mechanisms into sub-sources that only contain the corresponding partial spectrum. This step has to be carried out before the feature calculation, so the feature-set presented in this paper cannot be used to detect this behavior. Thus, we focus on an easily detectable characteristic that many source spectra with multiple mechanisms exhibit. We found that often, a spectrum scales at low frequencies over Strouhal number and at high frequencies over Helmholtz number or vice versa. Thus, there exist two different aeroacoustic mechanisms. We use this observation in the following to identify and separate the spectra accordingly.\\

Consequently, we cut each source spectrum into two sub-spectra and calculate the mean broadband self-similarity (see subsection~\ref{sec:similarity}) for four cases:
\begin{enumerate}
\itemsep-0.1em 
	\item For the Strouhal number at low and high frequencies.
	\item For the Strouhal number at low and the Helmholtz number at high frequencies. 
	\item For the Helmholtz number at low and the Strouhal number at high frequencies. 
	\item For the Helmholtz number at low and high frequencies.
\end{enumerate}
Figure~\ref{fig:Figure01} $c)$ shows the resulting mean self-similarity for different cut-frequencies for a slat / slat track source of the Do728. We calculate the Strouhal number cut-frequency using the mean Mach number $\text{St}=\text{He}/\langle M_i\rangle$. The global optimum of the four cases defines the optimal cut frequency and the frequency types of the sub-spectra. In this case, we achieve the optimal self-similarity when we use the Strouhal number at low frequencies (Figure~\ref{fig:Figure01} $a$, below the vertical black line) and the Helmholtz number at high frequencies (Figure~\ref{fig:Figure01} $b$ above the vertical black line). However, often it is not clear (even for a human) if the spectrum should be separated and a false positive separation has a greater impact on the feature calculation and clustering than a false negative separation. Hence, we prefer to leave a spectrum intact if the need for separation is unclear. We define a variety of rules that must be met before the source is separated into sub-sources. First, the overlapping spectra at different Mach numbers must cover at least two octaves to prevent small sub-spectra with little information. Second, the sub-spectra should both cover at least half an octave to prevent small, irrelevant spectra parts. Third, we only separate the source if the optimal similarity is achieved using a different scaling behavior at low and high frequencies. Forth, the mean self-similarity of the sub-spectra of different frequency-types must feature at least a $\SI{10}{\percent}$ improvement over the maximum mean self-similarity of the same frequency types. In the example of the slat / slat track, the first three rules are met, but the self-similarity improvement of around $\SI{7}{\percent}$ from $\text{He}_\text{cut}(\langle\text{St}_l,\text{He}_h\rangle)\approx14$ would not justify the spectrum separation, compared to sub-spectra with a Helmholtz number scaling at $\text{He}_\text{cut}(\langle\text{He}_l,\text{He}_h\rangle)\approx24$. The parameters for the rules are based on the presented data and can be adjusted to meet a more or less rigorous separation policy.

\begin{figure}
	\centering
	\includegraphics[width=\reprintcolumnwidth]{Figure01}
	\caption{(Color online) Do728, $\text{Re}=\SI{1.4e6}{}$, slat / slat track source at $\alpha=\SI{1}{\degree}$. $a)$ shows the spectra over Strouhal and $b)$ over Helmholtz number. The vertical black lines depict the optimal frequency to separate the spectra into low $l$ and high $h$ sub-spectra, to ensure their optimal self-similarity. In $c)$ the mean self-similarity (scal), see eq.~\ref{eq:scalability}, for the four possible combinations of Strouhal $\text{St}_{l,h}$ and Helmholtz number $\text{He}_{l,h}$ based on the depicted spectra cut-frequency on the x-axis are shown. The $x$ marks the global maximum, which leads to the spectra separation in $a)$ and $b)$. For this source, a Strouhal number scaling below $\text{He}\approx15$ and Helmholtz number scaling above this frequency achieves the optimal self-similarity of the sub-spectra.}
	\label{fig:Figure01}
\end{figure}



% In sub-section~\ref{sec:spectra_seperation} we showed that spectra often contain frequency intervals, that are governed by different physical mechanisms. While we observed most of the characteristic features at lower Strouhal numbers $\text{St}\le 100$, some sources showed a different behavior at high Strouhal numbers, see Figure~\ref{fig:Figure03}. For this, we identified the inner slat, slat / slat tracks, slat edge and the nacelle vicinity, see Figure~\ref{fig:Figure01}, Figure~\ref{fig:Figure03}, and Figure~\ref{fig:Figure07} $a)$, $j)$, $k)$ and $n)$. We showed that this behavior can be detected using the definition of the self-similarity over Strouhal and Helmholtz number from sub-section~\ref{sec:similarity}. We assumed that if a spectrum scales at low frequencies over Strouhal number and at high frequencies over Helmholtz number or vice versa, it must be governed by two different source mechanisms. Thus, the source spectra can be separated into sub-spectra that feature a single source mechanism, respectively. Since a false positive separation of a spectrum can lead to the insufficient calculation of aeroacoustic properties we introduced rules to ensure a conservative spectrum separation policy. The variables of these rules were based on the spectra of the presented datasets and should be reviewed for other data. The sources in our data showed mostly one or two different frequency regions, but more complex sources might be possible. Since we had to manually classify all individual sources for a ground truth and interpret the clustering results, we chose not to complicate the process by splitting spectra. However, the clustering results may be improved using this technique.\\
